Gummy Browsers: Targeted Browser Spoofing against State-of-the-Art Fingerprinting Techniques

We present a simple yet potentially devastating and hard-to-detect threat, called Gummy Browsers, whereby the browser fingerprinting information can be collected and spoofed without the victim's awareness, thereby compromising the privacy and security of any application that uses browser fingerprinting. The idea is that attacker A first makes the user U connect to his website (or to a well-known site the attacker controls) and transparently collects the information from U that is used for fingerprinting purposes. Then, A orchestrates a browser on his own machine to replicate and transmit the same fingerprinting information when connecting to W, fooling W to think that U is the one requesting the service rather than A. This will allow the attacker to profile U and compromise U's privacy. We design and implement the Gummy Browsers attack using three orchestration methods based on script injection, browser settings and debugging tools, and script modification, that can successfully spoof a wide variety of fingerprinting features to mimic many different browsers (including mobile browsers and the Tor browser). We then evaluate the attack against two state-of-the-art browser fingerprinting systems, FPStalker and Panopticlick. Our results show that A can accurately match his own manipulated browser fingerprint with that of any targeted victim user U's fingerprint for a long period of time, without significantly affecting the tracking of U and when only collecting U's fingerprinting information only once. The TPR (true positive rate) for the tracking of the benign user in the presence of the attack is larger than 0.9 in most cases. The FPR (false positive rate) for the tracking of the attacker is also high, larger than 0.9 in all cases. We also argue that the attack can remain completely oblivious to the user and the website, thus making it extremely difficult to thwart in practice.

==> abstract.tex <==

\begin{abstract}
%\vspace{-12mm}
%It is believed that several websites are using browser fingerprinting for the purpose of advertisement targeting\cite{ref8}. 

%20210617	Several web services might be using browser
%20210617	fingerprinting for various purposes, including targeted advertising, user
%20210617	authentication and fraud detection. Researchers have developed a myriad
%20210617	of browser fingerprinting techniques based on a variety of browser attributes,
%20210617	such as browser vendor and version, canvas rendering, fonts, GPU and graphic drivers, and browser plugins, that may remain unique to a browser over a period of time, uniquely identifying a browser with a high accuracy.
	%Variations of canvas fingerprinting is based on the variations of
	%devices GPU and graphic drivers\cite{ref56}. Different devices may
	%install different kinds of fonts, so the fonts list would be different
	%in different devices. The plugins fingerprinting is the plugins list
	%installed in the browser, and it depends on the personal plugin
	%configuration.


%In this paper, the browser fingerprinting information can be collected and spoofed by the attacker, with browser console and browser extension. 

%\vspace{-1mm}
%	In this paper,
	 We present a simple yet potentially devastating and hard-to-detect threat, called \textit{Gummy Browsers}\footnote{Named after ``Gummy Fingers'' that can impersonate a user's fingerprint biometrics.}, whereby
%	the browser fingerprinting information can be collected and spoofed without the user's awareness,
the browser fingerprinting information can be collected and spoofed without the victim's awareness,
	thereby compromising the privacy and security of any application that
	uses browser fingerprinting. The idea is that the attacker $A$ first
	makes the user $U$ connect to his website (or to a
	well-known site the attacker controls) and transparently collects the information from $U$ that
	is used for fingerprinting purposes (just like any fingerprinting
	website $W$ collects this information). Then, $A$
	orchestrates a browser on his own machine to replicate and transmit the
	same fingerprinting information when connecting to $W$, fooling $W$ to
	think that $U$ is the one requesting the service rather than $A$. As a consequence, if $W$ populates targeted ads for $U$ based on only browser fingerprints, $A$ can now start seeing the same or
% very
	similar ads on his browser as $U$ would see. This will allow the attacker to profile $U$ and compromise $U$'s privacy.
	%This can happen over a long period of time which
	%would allow $A$ to compile different ads that the $U$ is seeing,
	%thereby learning a wealth of potentially sensitive information about the
	%\textcolor{blue}{$U$} (as prior work on ad privacy shows).
	%Similarly, if $W$ uses \textcolor{blue}{only} fingerprinting for user authentication,
	%$A$ can impersonate as $U$. Likewise, if $W$ deploys fingerprinting
	%for fraud detection (e.g., to defeat clickbots) \textcolor{blue}{based on only fingerprinting techniques}, $A$ can bypass the detection
	%process.
	
%\vspace{-1mm}
We design and  implement the \GB\ attack using three orchestration methods
	based on script injection, browser settings and debugging tools, and
	script modification, that can successfully spoof a wide variety of
	fingerprinting features to mimic many different
	browsers (including mobile browsers and the Tor browser). We then
	evaluate the attack against two state-of-the-art browser fingerprinting
	systems, \textit{FPStalker} and \textit{Panopticlick}. Our results show
	that $A$ can accurately match his own manipulated browser fingerprint
	with that of any targeted victim user $U$'s fingerprint for a long
	period of time, without significantly affecting the tracking of $U$ and
	when only collecting $U$'s fingerprinting information only once. The
	TPR (true positive rate) for the tracking of the benign user in the
	presence of the attack is larger than 0.9 in most cases.  The FPR
	(false positive rate) for the tracking of the attacker is also high,
	larger than 0.9 in all cases.  We also argue that the attack can remain
	completely oblivious to the user and the website, thus making
	it extremely difficult to thwart in practice. 
	
	
%	The smallest TPR value of
%	Panopticlick and \HLA\ in our attack is larger than 0.85 under all
%	collect frequency, and most of values are larger than 0.9. The smallest
%	TPR value of \RLA\ in our attack is larger than 0.925 under all collect
%	frequency, and most of values are larger than 0.95. FPR of \HLA\ has
%	smallest value that larger than 0.925. 0.95. And this score for
%	Panopticlick and \RLA\ is 0.975 and 0.95. Most of values are larger
%	than 0.975, 1 and 0.95 in Panopticlick, \RLA\ and \HLA.


%The attack has broader implications. Since browser fingerprinting is also used for the purpose of fraud detection and user authentication, our attack can be used to bypass the security offered by these defensive applications of browser fingerprinting as well.
%\textcolor{blue}{Our experiments considered that the website only uses browser
%fingerprinting for user tracking, and did not use cookies (or that the cookies were blocked by the user), and therefore our
%attacks and implications of our attacks are only limited to 
%fingerprint only.}


\end{abstract}

%\vspace{-10mm}

==> tprfpr.tex <==
Figures [\ref{fig:2b} -- \ref{fig:20af}] shows TPRs in the benign setting, and TPRs and FPRs in the attack setting for different collect frequencies.

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign2.pdf}
    \label{fig:2b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign2.pdf}
    \label{fig:2b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign2.pdf}

  \label{fig:2b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 2}
	\label{fig:2b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr2.pdf}
    \label{fig:2at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr2.pdf}
    \label{fig:2at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr2.pdf}

  \label{fig:2at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 2}
	\label{fig:2at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr2.pdf}
    \label{fig:2af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr2.pdf}
    \label{fig:2af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr2.pdf}

  \label{fig:2af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 2}
	\label{fig:2af}
\end{figure*}



\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign4.pdf}
    \label{fig:4b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign4.pdf}
    \label{fig:4b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign4.pdf}

  \label{fig:4b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 4}
	\label{fig:4b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr4.pdf}
    \label{fig:4at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr4.pdf}
    \label{fig:4at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr4.pdf}

  \label{fig:4at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 4}
	\label{fig:4at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr4.pdf}
    \label{fig:4af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr4.pdf}
    \label{fig:4af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr4.pdf}

  \label{fig:4af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 4}
	\label{fig:4af}
\end{figure*}


\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign6.pdf}
    \label{fig:6b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign6.pdf}
    \label{fig:6b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign6.pdf}

  \label{fig:6b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 6}
	\label{fig:6b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr6.pdf}
    \label{fig:6at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr6.pdf}
    \label{fig:6at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr6.pdf}

  \label{fig:6at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 6}
	\label{fig:6at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr6.pdf}
    \label{fig:6af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr6.pdf}
    \label{fig:6af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr6.pdf}

  \label{fig:6af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 6}
	\label{fig:6af}
\end{figure*}


\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign8.pdf}
    \label{fig:8b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign8.pdf}
    \label{fig:8b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign8.pdf}

  \label{fig:8b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 8}
	\label{fig:8b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr8.pdf}
    \label{fig:8at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr8.pdf}
    \label{fig:8at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr8.pdf}

  \label{fig:8at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 8}
	\label{fig:8at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr8.pdf}
    \label{fig:8af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr8.pdf}
    \label{fig:8af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr8.pdf}

  \label{fig:8af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 8}
	\label{fig:8af}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign10.pdf}
    \label{fig:10b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign10.pdf}
    \label{fig:10b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign10.pdf}

  \label{fig:10b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 10}
	\label{fig:10b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr10.pdf}
    \label{fig:10at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr10.pdf}
    \label{fig:10at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr10.pdf}

  \label{fig:10at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 10}
	\label{fig:10at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr10.pdf}
    \label{fig:10af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr10.pdf}
    \label{fig:10af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr10.pdf}

  \label{fig:10af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 10}
	\label{fig:10af}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-benign20.pdf}
    \label{fig:20b1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-benign20.pdf}
    \label{fig:20b2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-benign20.pdf}

  \label{fig:20b3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the benign setting when collect frequency is set as 20}
	\label{fig:20b}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-tpr20.pdf}
    \label{fig:20at1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-tpr20.pdf}
    \label{fig:20at2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-tpr20.pdf}

  \label{fig:20at3}
}
	\caption{True positive rate (TPR) as a function of tracking days in the attack setting when collect frequency is set as 20}
	\label{fig:20at}
\end{figure*}

\begin{figure*}[]
	\subfloat[Panopticlick]{
  \includegraphics[width=.3\linewidth]{appendix_figure/pano-fpr20.pdf}
    \label{fig:20af1}}
  %\hfill
  \subfloat[\RLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/rule-fpr20.pdf}
    \label{fig:20af2}}
  %\hfill
  \subfloat[\HLA]{
  \includegraphics[width=.3\linewidth]{appendix_figure/hybrid-fpr20.pdf}

  \label{fig:20af3}
}
	\caption{False positive rate (FPR) as a function of tracking days in the attack setting when collect frequency is set to 20}
	\label{fig:20af}
\end{figure*}
